On the Efficacy of Text-Based Input Modalities for Action Anticipation

Anticipating future actions is a highly challenging task due to the diversity and scale of potential future actions; yet, information from different modalities help narrow down plausible action choices. Each modality can provide diverse and often complementary context for the model to learn from. While previous multi-modal methods leverage information from modalities such as video and audio, we primarily explore how text descriptions of actions and objects can also lead to more accurate action anticipation by providing additional contextual cues, e.g., about the environment and its contents. We propose a Multi-modal Contrastive Anticipative Transformer (M-CAT), a video transformer architecture that jointly learns from multi-modal features and text descriptions of actions and objects. We train our model in two stages, where the model first learns to align video clips with descriptions of future actions, and is subsequently fine-tuned to predict future actions. Compared to existing methods, M-CAT has the advantage of learning additional context from two types of text inputs: rich descriptions of future actions during pre-training, and, text descriptions for detected objects and actions during modality feature fusion. Through extensive experimental evaluation, we demonstrate that our model outperforms previous methods on the EpicKitchens datasets, and show that using simple text descriptions of actions and objects aid in more effective action anticipation. In addition, we examine the impact of object and action information obtained via text, and perform extensive ablations.

==> sections/intro.tex <==
\section{Introduction}
\label{sec:intro}
Suppose you go to a cafe and order a coffee and you see your barista steaming milk, can you predict what they might do next? 
Action anticipation is the task of predicting future actions, using visual cues and data from other modalities such as audio, sensor data, etc.\ from current and prior observations, as displayed in Figure~\ref{fig:template}. 
Predicting future actions is important for many Artificial Intelligence (AI) applications such as autonomous driving~\cite{jain2015car,rasouli2020pedestrian}, assistive robotics~\cite{petkovic2019human,koppula2015anticipating,korbar2018co}, augmented reality, etc.
For instance, a kitchen robot can preemptively chop onions and hand them over if it can anticipate that the recipe requires chopped onions to be added next.
\harish{can remove this last sentence, as it is an additional example. Or remove the first sentence. }

\begin{figure}[]
    \centering
    \includegraphics[width=1\columnwidth]{pics/Template.pdf}
    \caption{\textbf{Anticipating actions} $\tau_{a}$ seconds after observing information for $\tau_{o}$ seconds using multiple modalities.}
    \label{fig:template}
\end{figure}


Although seemingly straightforward for humans, this task is difficult for AI models due to the challenging nature of predicting the future, due to the wide range of possible actions that the models have to learn. 
Models not only have to detect the action happening at the observed time, but also fuse information from all available modalities to anticipate future actions.
To formalize this task, challenging large-scale datasets such as Epic-Kitchens and Ego-4D~\cite{damen2018scaling,damen2020rescaling,grauman2022ego4d,stein2013combining} have been developed, along with accompanying benchmarks, challenges, and leaderboards for state-of-the-art methods, for action anticipation, action recognition, action detection etc.


Typically, short- and long-term action anticipation involves extracting frame level features from videos and aggregating them using either temporal recurrent~\cite{furnari2019anticipating,furnari2020rolling} and attention modules~\cite{girdhar2021anticipative,zhong2023anticipative}, or directly extracting video level features using attention~\cite{girdhar2021anticipative,wu2022memsit,roy2023predicting,roy2021action}. 
While attention can be employed, action anticipation using only videos--a single modality--still remains challenging, and the availability of additional and complementary modalities is typically advantageous~\cite{girdhar2021anticipative,zhong2023anticipative}.

For example, if an assistive robot is performing a task with camera pointed away from the person, and the person falls, the robot should still be able to react in a timely manner \textit{if} audio is being used as an additional modality. 
Such scenarios demonstrate that information from multiple modalities can aid in many tasks, including action anticipation.
Accordingly, recent works ~\cite{zhong2023anticipative,girdhar2021anticipative,thakur2023enhancing} have shown that action anticipation greatly benefits from multi-modal training, as well as knowledge from other visual and audio cues such as active object detection, self-supervised future feature prediction, speech recognition, and hand-object contact information, typically by using modality specific encoders.
In contrast, we examine the necessity for training such \emph{modality-specific encoders}, and, instead aim to determine \emph{if natural language descriptions are effective for action anticipation.} 
Further, contrastive pre-training has also been employed for multi-modal setups where modality features are aligned with text, e.g., CLIP, X-CLIP~\cite{radford2021learning,ma2022x} and other foundation models~\cite{zhu2023languagebind,girdhar2023imagebind,wu2022memsit,ni2022expanding}. 

Therefore, we leverage language models to generate features by encoding object and actions in text, in lieu of relying on traditional feature extracting methods. 
Further, we also study which modalities are more beneficial and inspect how the accuracy of action recognition for the observed frames affects anticipation. 
One primary requirement for an effective contrastive learning protocol is training with large batches. 
However, in a limited training resource setup, we explore alternate ways of adding more samples during training, and explore other self-supervision through inter and intra modality contrastive learning. 
\apoorva{Need to rewrite this}

In this paper, we present `Multi-Modal Contrastive Anticipative Transformer (M-CAT)' that utilizes contrastive pre-training for generated captions from actions for videos. 
As Large Language Models (LLMs) are adept in giving long descriptions when prompted, we utilize this feature to generate long descriptions for actions that often involve additional knowledge on the environment and objects, e.g., kitchen vs living room, utensils used etc., allowing M-CAT to encode this knowledge aiding in action anticipation.
 
We employ a two-stage network that first learns to recognize actions by contrasting fused features from multiple modalities against text, and subsequently predicting future actions by training a single linear layer.

The first stage utilizes a CLIP-like framework which contrasts visual embeddings fused from multiple modalities against text embeddings, enabling our model to learn more descriptions for actions generated through GPT models.
In the second stage, these fused features are then used to anticipate actions by training a classifier.

In summary, our contributions are: 
\begin{itemize}
    \item We propose a novel training protocol for predictive video modeling by contrasting modality features against action descriptions generated using LLMs.
    \item We propose and analyze using modalities in text format (actions and objects as text) for predictive modeling, and show that text based inputs generate strong features.
    \item We introduce methods to improve contrastive pre-training for small batch size capabilities and also introduce additional self-supervision.
    \item We perform extensive analysis and ablations for different design choices, pre-training protocols and modalities used for our approach.
    \item We also conduct in-depth analysis on the affects of accurate action prediction for the observed frames.
\end{itemize}

\begin{figure}[!t]
    \centering
    \includegraphics[width=1\columnwidth]{pics/Overview_loss.pdf}
    \caption{\textbf{Left:} Overview of our architecture. we split the training into two stages. 
    In the first stage, contrastive training, we fuse embeddings from different modalities using a Fusion Module $\mathcal{F}$, followed by an anticipation module $\mathcal{B}$.
    The output is contrasted against the action descriptions generated from a LLM. 
    The second stage involves action anticipation, i.e., utilizing a linear layer to predict actions.
    \textbf{Right:} Illustration of the image-text and image-image contrastive loss.}
    \label{fig:overview}
\end{figure}
